NetShaper: A Differentially Private Network Side-Channel Mitigation System

The widespread adoption of encryption in network protocols has significantly improved the overall security of many Internet applications. However, these protocols cannot prevent network side-channel leaks -- leaks of sensitive information through the sizes and timing of network packets. We present NetShaper, a system that mitigates such leaks based on the principle of traffic shaping. NetShaper's traffic shaping provides differential privacy guarantees while adapting to the prevailing workload and congestion condition, and allows configuring a tradeoff between privacy guarantees, bandwidth and latency overheads. Furthermore, NetShaper provides a modular and portable tunnel endpoint design that can support diverse applications. We present a middlebox-based implementation of NetShaper and demonstrate its applicability in a video streaming and a web service application.

==> Makefile <==
PAPER = paper
TEX = $(wildcard *.tex src/*.tex)
BIB = paper.bib
FIGS =
PLOTS	=

.SUFFIXES: .plot .eps .fig .png .pdf

all: graphs figures $(PAPER).pdf

graphs: $(addprefix plots/, $(addsuffix .pdf, $(PLOTS)))

figures: $(addprefix figures/, $(addsuffix .pdf, $(FIGS)))

$(PAPER).aux: $(TEX)
	pdflatex $(PAPER).tex

$(PAPER).bbl: $(PAPER).aux $(PAPER).bib
	bibtex $(PAPER)

$(PAPER).pdf: $(TEX) $(PAPER).bbl
	pdflatex $(PAPER).tex
	pdflatex $(PAPER).tex

clean:
	rm -f *.aux *.bbl *.blg *.log *.out $(PAPER).pdf *.fdb_latexmk *.fls

BASE ?= 8d8a2
#BASE ?= sec24summer
#BASE ?= ee91ff3
HEAD ?= HEAD

BASE_SHORT ?= $(shell git rev-parse --short ${BASE})
HEAD_SHORT ?= --

# (1) clone https://gitlab.com/git-latexdiff/git-latexdiff
# (2) cd git-latexdiff && make && make install
# (3) run 'make diff BASE=<version you want to compare against>'
diff::
	git latexdiff --main ${PAPER}.tex --latexmk  \
		${BASE_SHORT} ${HEAD_SHORT} \
		-o ${PAPER}-diff.pdf \
		--ignore-latex-errors --view	\
		--exclude-safecmd="todo,update,am,as,ml,mis,cite,textcolor"


.PHONY: all clean


==> discussion.tex <==
\section{Limitations and Discussion}
\label{sec:discussion}

We discuss extensions of the {\sys}'s prototype to support additional usages.

\if 0
\paragraph{Multiplexing with non-sensitive flows}
%{\sys} currently assumes that the network paths of non-sensitive and sensitive
%flows are physically isolated. To overcome this limitation, {\sys} can integrate
To route non-sensitive flows alongside sensitive flows, {\sys} can integrate
TDMA (time division multiple access) scheduling \cite{vattikonda2012tdma,
beams2021ifs} in its architecture. Specifically, {\sys} must employ a
synchronous TDMA schedule on its ingress and egress ports and on its CPUs for
each traffic class. When the slot for non-sensitive flows is scheduled, the
traffic is simply routed from the {\sys}’s ingress port to the egress port and
vice versa without any modifications.
%
Note that each tunnel endpoint can use a different TDMA schedule. A synchronous
TDMA schedule between each pair of endpoints may be useful for minimizing
overheads but is not essential for end-to-end security guarantees.
\fi
%\subsection{Alternate deployments of {\sys}}

%\if 0
\textbf{Scheduling multiple tunnels.}
%When handling multiple tunnels, {\sys} must ensure that the
%unshaped traffic of one tunnel is not leaked to another tunnel. Such leaks may
%arise via contention side channels in the mdidlebox.
When handling multiple tunnels, the unshaped traffic of one tunnel could
indirectly affect the shape of traffic in another tunnel, thus potentially
leaking the traffic of the first tunnels.
%For this,
{\sys} must isolate the tunnels from each other in the middlebox.
%Based on \S\ref{sec:implementation}, we require that the {\prepare}
%and QUIC worker threads must be performance isolated from {\ushaper} in each
%tunnel, (ii) the timing of {\prepare} must be masked to secret-independent
%times.
{\sys} could partition the middlebox cores into three groups, each core group
hosting the {\ushaper} process, the {\prepare} threads, and the QUIC worker
threads from different tunnels.
Additionally, {\sys} must use a TDMA schedule among the {\prepare} threads,
while \update{padding} each thread's execution to a secret-independent time.
%In {\sys}, only the {\dshaper} components need to be isolated. {\sys} uses a
%TDMA to schedule the {\dshaper} processes of different tunnels.
Since each {\prepare} thread enqueues shaped buffers at secret-independent
times, QUIC workers of different tunnels can be scheduled to transmit
packets arbitrarily.
%can subsequently %package the buffers into packets and
%transmit the packets in their tunnels following any arbitrary schedule.
%
%{Determining optimal TDMA schedules and their adaptation to the changing
%number of active tunnels is left to future work.}
%\am{Not implemented, remove?}
%\fi

\textbf{Generalization to multi-node communication.}
%\todo{TODO: single application with multiple tiers (e.g., CDNs to serve
%    different parts of a web request) -- general DAG topology}
%\todo{TODO: multi-party communication (e.g., a group VoIP call relayed through a
%    central server) -- star topology}
%{\sys} mitigates network side channel leaks in bidirectional communications
%between a client-server pair. However, {\sys}'s DP shaping can be extended
Some applications may involve multiple nodes forming a communication graph,
where the communication graph could uniquely identify application secrets.
For example, dynamic web pages may be recognized from the traffic generated to
all servers hosting web page components.
%serving dynamic web pages may require downloading embedded objects from
%multiple  servers.
{\sys} can be extended to protect secrets in such applications.
{\sys}'s middlebox is portable and can be easily added in front
of each node to shape traffic on all links.
A client could establish tunnels among all pairs of nodes in an application for
the duration of its interaction with the application.
Each link could use its own DP parameters for shaping; the privacy
guarantees over the communication graph would be a composition of DP guarantees
of all links in the graph.
We leave a detailed analyses of privacy guarantees and overheads in a multi-node
application to future work.
%The key requirement is to model a ``buffering queue'' to define the maximum
%information that could be accessed by an adversary in the communication graph.

\textbf{Integrating {\sys} with end hosts.}
To ensure end-to-end security while accessing sensitive services from outside
organization premises, users could use a VPN client on their devices that is
enhanced with {\sys}'s shaping capabilities. A key challenge would be to ensure
performance isolation of the {\sys}-enhanced VPN client from the application
handling sensitive data \cite{mehta2022pacer}.

\textbf{Integrating {\sys} with other technologies.}
{\sys} can be considered as a network function (NF) and can be integrated with a
chain of other NFs, such as load balancers, firewalls, and intrusion-detection
systems. {\sys} could be the first function in an NF chain, interfacing with the
external network, which forwards inbound flows to other NFs after dropping
padding and shapes only select outbound flows forwarded by the next NF in the
chain. Placing {\sys} at the beginning of the chain would minimize the
communication bandwidth within the NF chain and the private network.
%\am{just mention as a one line somewhere earlier?}
%\paragraph{Interaction between {\sys} and DPI technologies.}
%{\sys} does not conflict with deep packet inspection (DPI) technologies, which
%an organization may use to monitor their inbound traffic for suspicious
%behaviors. However, {\sys} protects against third-party DPI which may


%\subsection{Generalization for orthogonal goals}
%\paragraph{Anonymity.}


==> dp.tex <==
\section{Differentially Private Traffic Shaping}
\label{sec:dp}

\if 0
\begin{algorithm}[t]
    \DontPrintSemicolon
    \SetNoFillComment
    % \KwIn{$S_N, Q, T, \varepsilon, w, D, min\_burstsize, max\_burstsize$}
    \SetKwFunction{get}{get\_dp\_size}
    \SetKwFunction{send}{send\_data}
    \SetKwFunction{dequeue}{dequeue}
    \SetKwFunction{doshape}{do\_shape}
    \SetKwFunction{addhdr}{add\_dp\_header}
    \SetKwFunction{encrypt}{encrypt}
    \SetKwFunction{sendpkt}{send\_udp\_pkt}
    \SetKwProg{Fn}{Function}{:}{}

    \Fn{\get{$Q,\; \varepsilon$}}{
        \am{where do $D_N$, $B_{min}$, $B_{max}$ come from?} \;
        $D^N = Q + \mathcal{N}(0, \sigma)$ \;
        $D^{N}_{clipped} =\max (B_{min}, \; \min (B_{max}, \; D_N))$ \;
        \textbf{return} $D^{N}_{clipped}$ \;
    }
    \Fn{\send{$len_R,\; len_D,\; MTU$}}{
        buf[0:$len_R$ -1] = \dequeue($Q_R$, $len_R$)\;
        buf[$len_R$:$len_R$ + $len_D$ -1] = \dequeue($Q_D$, $len_D$)\;
        \While{(buf.size $\neq$ 0)}{
            plen = buf.size > MTU ? MTU : buf.size\;
            pkt.payload = buf.get\_data(plen)\;
            buf.size -= sizeof(pkt.payload)\;
            \tcc{Header to track dummy data.}
            pkt.payload = \addhdr(pkt.payload)\;
            pkt.payload = \encrypt(pkt.payload)\;
            \sendpkt(pkt)\;
        }
    }
    \Fn{\doshape{}}{
        %\textbf{SendPacket}(queue\_state, pkt\_size, delay)\;
        \While{(not at end of data transmission)}{
            {sleep}($T$)\;
            $t$ = {get\_current\_time}()\;
            $Q_t$ = {get\_queue\_size}($t$)\;
            $D^S_t$ = \get($Q_t, \; \varepsilon$)\;
            $D^R_t$ = $\min (Q_t, D^S_t)$ \tcc{payload len}
            $D^P_t$ = $D^S_t - D^R_t$ \tcc{dummy len}
            \send$(D^R_t,\; D^P_t,\; MTU)$ \;
        }
    }
    \caption{Shaper logic}
    \label{alg:middle-box-all}
\end{algorithm}
\fi

% In this section, we describe our conceptual shaping strategy. In the next
% sections, we describe the design of our complete system that uses the strategy
% while shaping actual traffic.

Shaping involves transmitting packets such that their sizes and timing do not reveal secrets.
The goal of our DP traffic shaping mechanism is to dynamically adjust the data transmission rate based on the available data stream, all while ensuring that the DP guarantees hold for any information that an attacker, as defined in our threat model (\S\ref{subsec:threat-model}), can observe.
The design of our traffic shaping algorithm relies on three key steps.
%
First, we formalize the information available to an attacker observing an application stream, which is all information such as packet sizes or timing at the finest granularity of observation.
We propose to use a buffering queue to collapse all this information into a sufficient statistic to adapt {\sys}'s transmission rate: the size of data in the queue waiting to be transmitted through our shaping mechanism (\S\ref{subsec:infromation-bottleneck}).
%
Second, we show how to perform {\em DP measurements} of our buffering queue, in order to adapt \sys's transmission rate with DP guarantees.
Indeed, we show that under natural constraints on the transmission rate decision mechanism, the change of queue size is bounded, allowing us to perform DP measurements (\S\ref{subsec:dp-queue-measurements}).
%
Third, we describe our decision mechanism for sending data based on DP decisions, which completes our DP shaping mechanism (\Cref{alg:dp_shaping_mechanism}).
Intuitively, we can use DP queue measurements and public information such as network conditions to decide the amount of data to transmit.
Transmissions contain queued data when some is available, and dummy data otherwise.
The stream observed by any attacker is a post-processing of the DP queries issued on the queue (depends on the private data only through the DP measurements), and is hence DP.


% Our key insight is that the size of data waiting to be transmitted in our shaped
% tunnel is a sufficient statistic to adapt \sys's transmission rate.
% %
% by decapsulating \ml{?} packets and buffering content,
% we can make adaptive decisions on
% make adaptive decisions on this state, and only adapt to the data based on these measurements. We can then use the post-processing guarantee)
% We rely on periodic transmission intervals of constant lengths, while ensuring
% that the number of bytes transmitted within each interval is noised according to
% our differential privacy strategy.
% %
% The differentially private strategy relies on composition
% theorem~\citeme{dp-composition}. Specifically, we model an application
% stream as a sequence of windows of packet transmissions and reason
% about per-window linkage and accumulation of leakage over multiple
% windows.

% In the following, we provide a formal definition of differentially privacy in
% traffic shaping and then describe how we use it to shape application traffic
% streams.


% \label{subsec:infromation-bottleneck}
% \begin{figure}[t]
%   \centering
%   %  \includegraphics[width=\columnwidth]{figures/Design_highlevel.pdf}
%   %  \includegraphics[width=\columnwidth]{figures/minesvpn-overview-half.pdf}
%   %  \includegraphics[width=\columnwidth]{figures/minesvpn-arch4.pdf}
%   \includegraphics[width=\columnwidth]{figures/DPshaping_concept_horizontal.pdf}
%   \caption{{\sys} overview (one tunnel endpoint)
%       %\am{Update figure}
%   }
%   \label{fig:DPshaping_concept_horizontal}
% \end{figure}

\begin{figure}[t]
  \centering
  %  \includegraphics[width=\columnwidth]{figures/Design_highlevel.pdf}
  %  \includegraphics[width=\columnwidth]{figures/minesvpn-overview-half.pdf}
  %  \includegraphics[width=\columnwidth]{figures/minesvpn-arch4.pdf}
  \includegraphics[width=\columnwidth]{figures/DPshaping_concept_vertical.pdf}
  \caption{{\sys} traffic shaping stages}
  \label{fig:DPshaping_concept_vertical}
\end{figure}

\subsection{DP shaping building blocks}
\label{subsec:infromation-bottleneck}
We define a source application stream $S$ (i.e. the input stream) as a sequence of packets:
\begin{equation}\label{equ:stream-pkts}
        S = \{P_{t_1}^S, P_{t_2}^S, P_{t_3}^S, \dots \} ,
\end{equation}
where $P_{t_i}^S$ is the size of the packet transmitted as a part of the stream
$S$ at the time $t_i$. \am{The symbol $S$ is overloaded in many places.}\as{all of them referring to the input stream}
%\am{I realize this model is inaccurate. A more accurate description is that an
%application byte stream is transformed into a sequence of packets. In absence of
%shaping, packet sizes and timing reveal the secrets. {\sys} transforms an {\em
%application byte stream} into a sequence of DP shaped bursts that are
%transmitted within fixed intervals. Basically, DP does not get an input as a
%packet stream but rather as a byte stream.}
%
Without {\sys}'s shaping, an eavesdropper can observe the entire stream:
$S = \{P_{t_1}^S, P_{t_2}^S, P_{t_3}^S, \dots \}$.
Typically, this information is strongly correlated with the data sent by the
application and the eavesdropper can infer sensitive information, such as the
specific video being sent by a streaming
application~\cite{schuster2017beautyburst}.


% We start by modeling an application stream in one direction as a
% dataset of packet sequences and by defining neighboring datasets from
% application streams.

% %\Cref{fig:minesvpn-arch} represents the abstracted design of the {\sys}
% %middle-box.  The incoming traffic in \Cref{fig:minesvpn-arch} is in form of
% %packets.  We formalize a stream of traffic, $S$, with the following
% %representation:

% %\smallksip\noindent
% \paragraph{Input stream.}
% We model an application stream, $S_I$ as a sequence of packets
% %$\{P_{t_1}^S, P_{t_2}^S, P_{t_3}^S, \dots \}$,

% \begin{equation}\label{equ:stream-pkts}
        % S_I = \{P_{t_1}^S, P_{t_2}^S, P_{t_3}^S, \dots \}
% \end{equation}
% where $P_{t_i}^S$ is the size of the packet transmitted as a part of the stream
% $S$ at the time $t_i$.

%leading to information leakage \cite{beautyburst} \todo{More
%references are needed}.
%{\sys}'s {\DPlogic} decides {\em how many bytes} of data to enqueue into DP
%queue and {\em when} to enqueue them, which we collectively call DP
%mechanism.

%\ml{\am{Aastha} I feel like the DP section would be easier to digest
%if it came after the design section.}
In {\sys}, we first introduce an information bottleneck in the form of a
buffering queue, {$\unshapedQ$}, to control the information accessible by an
eavesdropper. The buffering queue has three operations: \texttt{enqueue(size)},
\texttt{dequeue(size)}, \texttt{get\_size()}.
Conceptually, {\sys} decapsulates all application traffic of incoming stream $S$, and enqueues it in the {$\unshapedQ$}.
The shaping mechanism in {\sys} periodically retrieves the queue size and determines the amount of data to dequeue from $\unshapedQ$ in order to transmit it as shaped traffic.
The shaped traffic is encapsulated into a new sequence of packets, which we
denote as:
\begin{equation}\label{equ:stream-segs}
  O = \{P_{t_1}^O, P_{t_2}^O, P_{t_3}^O, \dots\}
\end{equation}
where $P_{t_i}^O$ is a packet sent in the shaped tunnel.

In order to ensure that the observable stream $O$ preserves the privacy of the
original stream $S$, {\sys} ensures that $O$ is Differentially Private.
To enforce DP, {\sys} ensures that any input to $O$ that depends on sensitive
data (the stream $S$) is measured with DP. \am{Are we using $O$ for anything
other than just referring to the output packet sequence in the text and in the
diagram? This notation does not seem necessary for the rest of the section.}
\as{O just refers to the output (DP) packet sequence both in text and in diagram. Mathias used the $O$ for the output packet sequence and I didn't change the notation. }
\Cref{fig:DPshaping_concept_vertical} shows the end-to-end traffic shaping of
{\sys}.
After decapsulating incoming packets, the incoming traffic is stored in a
buffering queue. In fixed periods of length $T$, the \texttt{dequeue} operation is performed,
ensuring that the timing of the outgoing traffic remains independent of the
incoming traffic. 
We refer to $T$ as the length of update interval.
The size of the \texttt{dequeue} is determined by our
differential privacy mechanism, guaranteeing that the size of the outgoing
traffic remains DP.
Furthermore, the encapsulation and packetization of outgoing data can be
characterized as a post-processing step of a differentially private mechanism,
and therefore is DP.



%\am{If we agree
%about the model from byte stream to packet stream (unshaped) and burst stream
%(shaped), then this section can simply go away. The notion of shaping byte
%stream into a DP burst stream is already mentioned in the paragraph ``Traffic
%shaping within a tunnel'' in \S\ref{subsec:design-overview} currently. The only
%remaining abstraction is that of the queue. Do we need to introduce that in
%\S\ref{subsec:design-overview}?}

%\ml{$\leftarrow$ section where we show our attacks}

% \paragraph{Observed stream.}
% We define an observed stream $S_O$ as a sequence of bursts
% %transmitted at intervals of $T$
% %$\{B_1^S, B_2^S, B_3^S, \dots\}$,
% \begin{equation}\label{equ:stream-segs}
  % S_O = \{B_1^S, B_2^S, B_3^S, \dots\}
% \end{equation}
% where $B_i^S = \sum_{t_j \in [T_{i-1}, T_i]} P_{t_j}^S$ is the amount of traffic
% received between time intervals $T_{(i-1)}$ and $T_i$.
% Here, $T$ determines the granularity of attacker's observation.
% In absence of traffic shaping, an attacker can observe $S_O$ with high
% granularity and, if $S_O$ is correlated with secrets, can infer the
% secret~\cite{beautyburst}.
% %Our differentially private traffic shaping strategy ensures that the attacker is
% %not able trace back any traffic pattern transmitted over a public network to its
% %original pattern. This is achieved by shaping the traffic stream such that any
% %neighboring set of traffic streams has an equal probability of producing the
% %observed pattern. We will elaborate on our definition of neighboring streams in
% %the next section.

\subsection{DP queue measurements}
\label{subsec:dp-queue-measurements}
We define the queue $\unshapedQ_{\tau}$ as the size of {$\unshapedQ$} at time $\tau$.
To measure $Q_\tau$ with $(\varepsilon, \delta)$-DP, {\sys} uses an additive Gaussian noise mechanism.
That is, it computes $\tilde{Q}_\tau \triangleq Q_\tau + z$, where the noise $z$
is sampled from a normal distribution with a variance that depends on the DP
parameters and the sensitivity $\Delta$: $z \sim \mathcal{N}\big(0, \sigma^2 =
\frac{2\Delta}{\varepsilon}\ln(\frac{1.25}{\delta})\big)$.
Intuitively, the sensitivity $\Delta$ represents the size of a change in traffic
against which we quantify DP guarantees. Combining all of these elements, \Cref{alg:dp_shaping_mechanism} presents a simple pseudo-code for traffic shaping in {\sys}.
% \begin{algorithm}[h]
%   \While{not at end of data transmission}
%   {
%       $\unshapedq_{\tau}$ = \texttt{get\_size()} \;
%       $\tilde{\unshapedQ}_{\tau}$ = $\unshapedQ_{\tau} + z$ \;
%       \texttt{dequeue($\tilde{\unshapedQ}_{\tau}$)} \;
%       \texttt{sleep($T$)}
%   }
%   \label{alg:dp_shaping}
%   \caption*{{\sys} traffic shaping}
% \end{algorithm}

\begin{algorithm}[t]
  \caption{{\sys} DP traffic shaping}
  \label{alg:dp_shaping_mechanism}
  \begin{algorithmic}[1]
  \While {\textbf{not} end of data transmission}
    \State $\tau$ = \texttt{current\_time()}
    %
    \State $\unshapedQ_{\tau}$ = \texttt{get\_size()}
    %
    \State $\tilde{\unshapedQ}_{\tau}$ = $\unshapedQ_{\tau} +
    \mathcal{N}\big(0, \frac{2\Delta}{\varepsilon}\ln(\frac{1.25}{\delta})\big)$ \;
    %
    \State \texttt{dequeue($\tilde{\unshapedQ}_{\tau}$)}
    \State \texttt{sleep($T$)}
  \EndWhile
  \end{algorithmic}
\end{algorithm}



As we can see, the Gaussian noise is scaled to $\Delta$, so protecting traffic
that can change by larger amounts requires more noise to be added.
In DP, the sensitivity $\Delta$ is defined as the worst-case change of our
measurement $Q_\tau$, when changing one stream going through {$\sys$}.
To formalize this notion, we first need to define what changing one stream means.
In DP, this is done through a neighboring definition, which defines the
protection unit for our DP mechanism:

\begin{definition}
\label{def:neighboring-streams}
Consider two streams, $S$ and $S'$, being transmitted within a window of duration $w_s$. We define them as neighbors if
\begin{equation}\label{equ:stream-neighboring}
  \|S_t - S'_t\|_1 \leq D_s \; (bytes)
\end{equation}
%\ml{we probably need $w_S$ here or something, as we now have a protection window
%by assumption/design or dropping queues without anything sent for too long, and
%a measurement window by assumption of length}
%\as{I think we can just mention the $w_s$ here as a requirement/assumption, and
%then in design section, we say we'll enforce this assumption by dropping the
%data after $w_s$ seconds. Dropping the data to me is more like a design decision
%as it is not the only option to enforce this requirement. In an "imaginary"
%scenario, we can assume applications terminate their connections after $w_s$
%seconds of delay and there is no need to assume that the traffic can
%accumulate.}:

\end{definition}

That is, $S$ and $S'$ are neighbors if the L1-norm of their difference is less than $D_s$ on the time window of size $w_s$ (both $D_s$ and $w_s$ are parameters).
%
We utilize the L1-norm as our distance metric to quantify the dissimilarity
between two traffic streams, as it captures differences in both segment size and
temporal pattern.
%
Intuitively, {$\sys$} aims to ensure that a stream $S$ is indistinguishable (in the DP
sense) from a neighboring stream $S'$ by observing the shaped traffic.

Based on \Cref{def:neighboring-streams}, we can define the sensitivity $\Delta$ as the maximum
difference in {$\unshapedQ$} size at any time, had we changed stream $S$ from
any neighboring stream $S'$:
\begin{equation}
  \Delta = \max_{\tau}\max_{S, S'} | Q_{\tau} - Q'_{\tau} | .
\end{equation}

A key feature of $\sys$'s design is to ensure that the amount of data in a queue
can only change by at most $D_s$ when changing a stream $S$ by a neighboring
$S'$. We elaborate on this in \Cref{sec:design}.
Formally, {$\sys$} offers the following guarantee:
\begin{proposition}\label{prop:sensitivity}
  {$\sys$} enforces $\Delta \leq D_s$.
\end{proposition}
\begin{proofsketch}
  The proof relies on the following properties of {$\sys$}.
  Within windows of $w_s$ seconds, if $Q'_{\tau} > Q_{\tau}$, for the same noise draw $z$, $\tilde{Q}'_{\tau} > \tilde{Q}_{\tau}$, and \Cref{alg:dp_shaping_mechanism} sends at least as much data under $Q'_{\tau}$ as under $Q_{\tau}$, but not more than $\tilde{Q}'_{\tau} - \tilde{Q}_{\tau}$.
  Hence, $|Q'_{\tau+1} - Q_{\tau+1}| \leq |Q'_{\tau} - Q_{\tau}|$ and queues only get closer by \Cref{alg:dp_shaping_mechanism}, and only grow apart by the difference between $S$ and $S'$.
  The formal proof is in Appendix \ref{appendix:dp}.
\end{proofsketch}

Therefore, the accumulated difference between $S$ and $S'$ is upper-bounded by $D_s$.
This bound on the sensitivity of {$\unshapedQ$} over neighboring streams enables {$\sys$} to provide $(\varepsilon_{w_s}, \delta_{w_s})$-DP guarantees for shaped traffic stream observed for a given time window $w_s$. Formally, we have that:
\begin{proposition}\label{prop:dp}
  {$\sys$} enforces $(\varepsilon_{w_s}, \delta_{w_s})$-DP, with
  $\varepsilon_{w_s}, \delta_{w_s} \triangleq \textrm{DP\_composition}(\varepsilon,
  \delta, \lceil\frac{w_s}{T}\rceil)$.
\end{proposition}
\begin{proof}
By \Cref{prop:sensitivity}, the sensitivity of one {$\unshapedQ$} is $\Delta$. Every $T$ seconds, by the Gaussian mechanism the observed queue size, $\tilde{\unshapedQ}_{\tau}$, is $(\varepsilon, \delta)$-DP.
Over a time period of length $w_s$, there are at most $\lceil\frac{w_s}{T}\rceil$ measurements taken. The proof is then concluded by applying DP composition.
\end{proof}

Given the privacy parameters, $\varepsilon$ and $\delta$, for one queue measurement, and the number of measurements, $\lceil\frac{w_s}{T}\rceil$, the  $\textrm{DP\_composition()}$ uses RDP composition to calculate the aggregated privacy loss, $\varepsilon_{w_s}$, and failure probability, $\delta_{w_s}$, for the time window of $w_s$.
If $w_s$ is larger than any traffic stream to protect, {$\sys$} enforces $(\varepsilon_{w_s}, \delta_{w_s})$-DP over all streams going through he shaped tunnel. Note that this does not depend on the number of streams: the overhead (noise added to measurements) is the same regardless of how many streams use the shaped tunnel.




% \paragraph{Unshaped queue.}
% We model an abstract queue, {$\unshapedQ$}, which holds the unshaped input byte
% stream of an application and supports two operations: enqueue and dequeue.

% \paragraph{Neighboring queue states.}
% We define the queue state, ${\unshapedQ}_{\tau}$, as the amount of traffic
% inside ${\unshapedQ}$ at time $\tau$. We call two queue states, ${\unshapedQ}_{\tau}$
% and ${\unshapedQ}'_{\tau}$, neighbor queue states if and only if we have:
% \begin{equation}\label{equ:queue-neighboring}
        % |{\unshapedQ}_{\tau} - {\unshapedQ}'_{\tau}| \leq D_q \;(bytes)
% \end{equation}
% where $D_q$ is a parameter in our system.


% \paragraph{Query function and sensitivity.}
% We define a query function on the queue state ${\unshapedQ}$,
% $f({\unshapedQ}_{\tau})$, as a function that returns the
% size of the queue at time ${\tau}$. The sensitivity of the function $f$ is given~by:
% \begin{equation}
% \Delta_1 f = \max_{Q, Q'} \| f(Q_{\tau}) - f(Q'_{\tau}) \|_1 =  \max_{Q, Q'} \| Q - Q' \|_1 = D_q
% \end{equation}
% Here, $\Delta_1 f$ captures the magnitude by which the size of queue can change
% from one stream to another.  In fact, {\sys}'s shaping strategy guarantees that
% the queue size cannot be accurately ascertained by an attacker.  At this point,
% we have all necessary building blocks to propose our differentially private
% shaping algorithm.

% \paragraph{From queues to traffic streams.}

% The definition presented in \Cref{equ:queue-neighboring} serves as a sufficient
% basis for designing our differentially private traffic shaping based on queue
% states.  However, in order to provide comprehensive privacy guarantees for
% internet applications, we extend this definition from queue states to
% streams of traffic.


% To reason about the privacy of traffic streams, we need to define neighboring
% streams (i.e. the minimal protection unit of each differentially private
% algorithm).  Two stream prefixes, $S_t$ and $S'_t$ (with the representation of
% \Cref{equ:stream-segs}), are neighbors if and only if:
% \begin{equation}\label{equ:stream-neighboring}
        % \|S_t - S'_t\|_1 \leq D_s \; (bytes)
% \end{equation}
% We utilize the L1-norm as our distance metric to quantify the dissimilarity
% between two traffic streams, as it captures differences in both
% segment size and temporal pattern.


% Our goal is to measure, and subsequently bound, the privacy loss of a traffic
% stream.
% Intuitively, an attacker's observation of a traffic stream can be interpreted as
% a series of differentially private queries on the segment sizes of original
% traffic pattern. \am{I find this intuition of an attacker issuing DP queries
% strange. To me, the attacker performs usual queries on a database whose
% underlying distribution has been made DP.}
% We claim that the privacy loss for a individual traffic stream shaped with our
% mechanism can be quantified by aggregating the privacy loss incurred at each
% measurement of the abstract queue size.
% The following statement provides a formal representation of this notion.


% \ml{Amir, please use real latex things for the Claim and Lemma. I'd also call the Lemma Proposition instead: Lemma is for general theoretical tools others might reuse and apply to other proofs).}
% \textbf{Claim}: The privacy loss of transmitting a traffic stream with the
% length of $w = kT$ through the {\sys} middle-box, is the composition of $k$
% queries on the queue state.
% \\
% To show that this claim is true, we only need to prove the following lemma.

% \textbf{Lemma}: Assume two neighboring traffic streams, $S_t$ and $S_t'$,
% transmitted through a middle-box with \Cref{alg:middle-box-all} as the shaping
% mechanism. If they both reshaped to the same traffic stream, $S_O$, then,  at
% any given time $\tau$, the queue states for neighboring streams are $D$-close.
% In other words we have:
% \begin{equation}\label{equ:composition_dp_section}
        % \forall \tau > 0 : |Q_{\tau} - Q_{\tau}'| \leq D
% \end{equation}
% where $D = \min(D_q, Q_{max})$. $D_q$ and $Q_{max}$ are the queue neighboring
% threshold and maximum buffer size of our middle box respectively.
% \am{I see no relation between $D_q$ and $D_s$.}

% This means the unshaped queues of these two streams are always neighbors
% according to the neighboring definition of \Cref{equ:queue-neighboring}.
% We prove the Lemma in \Cref{appendix:dp}.

% Here, we show how we can calculate privacy loss for a traffic stream.
% Assume two neighbor streams, $S_t$ and $S_t'$, reshaped to the same stream,
% $S_O$, by {\sys} middle-box. If we show the shaping mechanism by $M_s$, the
% privacy loss is:
% \begin{equation}\label{equ:privacy-loss}
  % \log\big(\frac{\Pr[M_s(S_t)=S_O]}{\Pr[M_s(S_t')=S_O]}\big) \leq \varepsilon_g
% \end{equation}
% Using the representation of \Cref{equ:stream-segs}, we have:

% \todo{Add the equation}

% The composition comes into the picture in the inequality \todo{Add ref} as the
% size of output at each round depends on the amount traffic enqueued into the
% ${\unshapedQ}$ and outputs of previous rounds of the mechanism, which both
% abstracted in the queue state.

\if 0
\subsection{DP shaping mechanism}
\label{subsec:dp-shaping}

\ml{I feel like this all belong to \am{design} with the DP call as a noisy black
box.} \am{Yes, this is covered in \S\ref{subsec:design-overview}.}

\Cref{alg:middle-box-all} represents the differentially private shaping
mechanism.  The algorithm is executed periodically with an interval of $T$
seconds.  Here, we explain one round of the algorithm.
\begin{enumerate}
  \item The DP mechanism reads the current size of the queue, $Q_t$.
  \item Then, it adds a noise from a Gaussian distribution with an average of
  zero and scale of ${\sigma}$ to the current size. The noisy measurement is
  represented by $D^S_t$ in the algorithm, and $\sigma$ is the parameter that
  determines the privacy loss of our mechanism.
  \item To avoid unpredictable behaviors such as the occurrence of negative
  values in the noisy measurement, we have incorporated a minimum and maximum
  size threshold for the noisy measurements, which are adjustable parameters
  within the algorithm.
  \item If $D^S_t > Q_t$, the data in {\unshapedQ} will be padded to $D^S_t$
  bytes and subsequently transmitted to the receiver.
  Conversely, if the size of the data in {\unshapedQ} is less than or equal to
  $D^S_t$, the entirety of the $D^S_t$ bytes will be sent.  In algorithm
  \ref{alg:middle-box-all}, the padding size and real data size are represented
  with $D^P_t$ and $D^R_t$ respectively.
\end{enumerate}
\fi

Our algorithm ensures that an attacker cannot trace the observed segment sizes
on the network back to the original traffic pattern.  Furthermore, due to the
periodic execution of the algorithm, the timings of segments are independent of the
original pattern.

\am{The proof of the DP guarantees of the algorithm is provided in the
appendix. Can we prove that constant timing intervals + differentially privacy
on size = differentially privacy on the overall traffic shape?}

==> implementation.tex <==
\section{Implementation}
\label{sec:implementation}

\begin{figure}[t]
    \centering
    \includegraphics[width=\columnwidth]{figures/middlebox-arch.pdf}
    %    \includegraphics[width=\columnwidth]{figures/design.pdf}
    \caption{{\sys} middlebox design}
    \label{fig:minesvpn-impl}
\end{figure}

We present a middlebox based {\sys} implementation,
as shown in \Cref{fig:minesvpn-impl}.
%
Recall from \S\ref{subsec:key-ideas}, a middlebox can support shaping for
several applications and amortizes~the shaping cost among multiple flows that
share the same tunnel.
Moreover, middleboxes can support multiple ``long-term'' tunnels between
endpoints. Such tunnels may be set up, for instance, between organization
campuses to secure all communication between the campuses without the need for
modifying individual end hosts.

%\begin{table}[t]
%    \centering
%    \renewcommand{\arraystretch}{1.2}
%    \begin{tabular}{lll}
%        \toprule
%        {\bf Outer/Inner} & {\bf TCP} & {\bf UDP}
%        \\
%        \midrule
%        {\bf TCP} & meltdown & inefficient
%        \\
%        {\bf UDP} & insecure & OK
%        \\
%        \bottomrule
%    \end{tabular}
%    \caption{Impact of tunneling a transport inside transport}
%    \label{tab:transport-in-transport}
%\end{table}
%
Following the proxy architecture, the middlebox splits the communication between
two application endpoints over three transport connections:
one between two middlebox endpoints that provides a tunnel and one between
each application endpoint and its local middlebox.
In our implementation, a middlebox consists of two userspace processes,
{\ushaper} for unshaped traffic and {\dshaper} for shaped traffic,
which can run on any standard operating system kernel
and transport stack.
%For each tunnel supported by the middlebox, there is one {\dshaper} process. The
%{\ushaper} process simply multiplexes the flows mapped to all tunnels using one
%or more threads.
Together, the two processes mediate traffic between the application endpoints
and the middleboxes, and sending/receiving shaped traffic to/from the tunnel.
%{\sys}'s prototype relies on a Linux kernel with the standard TCP and UDP
%stack, and the MSQUIC implementation of the QUIC protocol.
%Together the two processes implement the following functionalities: (i)
%establishing tunnels with remote middleboxes, (ii) managing communication
%between local and remote application end points, (iii) moving traffic between
%local application endpoints and the tunnel, (iv) shaping tunnel traffic, and (v)
%providing end-to-end reliable delivery semantics.
We describe each {\sys} component and
how they ensure secret-independent shaping
both within one tunnel and then across multiple tunnels.

\if 0
\subsection{\todo{Middlebox-Middlebox Tunnel Setup}}

%Specifically, the {\dshaper} establishes tunnels with remote middleboxes, shapes
%the outbound traffic on each tunnel according to the tunnel's DP parameters, and
%handles inbound shaped traffic received from the tunnels. The {\ushaper} manages
%the connection with a local application endpoint and mediates the traffic
%between the application endpoint and the {\dshaper}.

%To protect an application's traffic, the middlebox must be placed inside the
%same private network as the application, so that the adversary cannot observe
%the traffic between an application and the middlebox.

%To establish an end-to-end connection, {\sys} relies on three piecewise
%transport connections: one between the two middlebox endpoints that provide a
%tunnel for the application endpoints, and one each between each application
%endpoint and its local middlebox endpoint.

%Each middlebox consists of two userspace processes: a {\ushaper}, which
%interfaces with the local application, and a {\dshaper}, which interfaces
%with the remote middleboxes.
%For each application flow handled by the middlebox, the {\ushaper} mediates
%establishment of the end-to-end connection between the application endpoints,
%and the sending and receiving of traffic from the associated tunnel.
%For this, the {\ushaper} maintains a set of a TCP socket, and a pair of
%transmit and receive queues.
%each application flow to its associated tunnel, sockets, and a pair of transmit
%and receive queues.

%The {\ushaper} shares with the {\dshaper} a {\flowmap} table containing
%mappings of the segments of end-to-end connections, a set of per-flow transmit
%queues, and a set of per-flow receive queues. Together, the two processes manage
%traffic flows on the end-to-end connections.

%\subsection{Shaping Components}
%{\sys} consists of two userspace processes, {\ushaper} and {\dshaper},
%which can run on top of any standard operating system and network stack. The
%{\ushaper} interfaces with the local application endpoints while the {\dshaper}
%process interfaces with the remote middleboxes of the tunnels it handles. The
%{\ushaper} shares the {\flowmap} table, a set of per-flow transmit queues,
%and a set of per-flow receive queues with the {\dshaper}.

%{\sys}'s basic proxy functionality includes setting up a connection between a
%middlebox pair that would carry shaped traffic for sensitive flows, setting up
%and tearing down a connection between the application endpoints for the
%sensitive flows, and  handling congestion. We describe these next.

%\am{de-duplicate from section 5.2, paragraph ``Traffic shaping within a
%    tunnel''.}
%For each tunnel interfacing with a remote middlebox, the {\dshaper}
%maintains a set of a QUIC socket, and a pair of threads, namely {\em Shaper}
%and {\em Shaped\-Receiver} threads.
%For each tunnel interfacing with a remote middlebox, the {\dshaper}
%maintains a set of a QUIC socket, and a pair of threads, namely {\em Shaper} and
%{\em ShapedReceiver}. The Shaper handles outbound traffic while the
%ShapedReceiver handles inbound traffic.


%\paragraph{Middlebox-middlebox tunnel setup.}
A {\sys} middlebox is statically configured with the addresses of the local
application hosts as well as other middleboxes to which the applications’
traffic must be forwarded\footnote{In practice, the middleboxes could discover
other middleboxes using DNS or similar protocols.}.
The {\dshaper} establishes QUIC tunnels with every remote middlebox specified in
its configuration.
%Each tunnel is identified by a 6-tuple consisting of the IP addresses and ports
%of source and destination middleboxes, a reliability flag, and a privacy
%descriptor.
%%{source middlebox IP, destination middlebox IP, source middlebox port,
%%destination middlebox port, reliability flag, privacy descriptor}.
%The reliability flag indicates if the tunnel provides reliable delivery
%semantics or not. The middlebox uses a reliable tunnel for shaping the traffic
%of applications using reliable transport (\eg TCP) and an unreliable tunnel for
%applications using unreliable transport (\eg UDP).
%The privacy descriptor indicates the DP configuration for the tunnel. All
%application flows passing through the same tunnel are subject to the same DP
%parameters.

After a QUIC connection is established between a pair of middleboxes, the
{\dshaper} process in each middlebox initializes three QUIC streams: a control
stream, a dummy stream, and a data stream.
%\todo{fixed number of data streams} that are used to carry the payload of
%application flows.
%The control and dummy streams are designated special stream IDs.
The control stream is used to transmit control messages related to establishment
and termination of the data stream that will subsequently transmit data in the
tunnel. The dummy stream is used to transmit padding in QUIC packets in the
form of QUIC STREAM frames.
%\am{mention reliance on QUIC's encryption protocol.}

%Once a tunnel has been established, each middlebox continuously transmits dummy
%packets at a uniform low rate in the tunnel. \am{Is it uniform as in constant
%shaping or DP shaped? How are we accounting for this overhead?}
%For this, the middlebox establishes a QUIC stream with a special ID, designated
%as the dummy stream, and generates STREAM frames of appropriate length.

\subsection{\todo{End-to-End Connection Management}}
When one application endpoint (\eg A1 in \Cref{fig:minesvpn-impl}) initiates
communication with another application endpoint (B1), the middlebox close to the
initiator (M1) and the responder (M2) work like a forward proxy and a reverse
proxy, respectively.
Together the two middlebox proxies establish a piecewise connection between the
application endpoints.

%\am{Compress to say, connection establishment like a standard forward and
%reverse proxy style.}
%Without loss of generality, we describe the the end-to-end connection
%establishment and termination in the context of a single-client-single-server
%application with one middlebox in front of each (cf.
%\Cref{fig:minesvpn-impl}).  The middleboxes in front of the client and the
%server are called the client middlebox and the server middlebox, respectively.
%
%A flow between a client and a server is carried through a connection that
%consists of three segments: (i) between the client and its middlebox, (ii)
%between the server and its middlebox, and (iii) between the client middlebox and
%the server middlebox. The {\ushaper} in the client middlebox intercepts the
%connection handshake messages from the client and notifies the {\dshaper}.
%The {\dshaper} in the client middlebox sends a handshake message to its peer
%in the server middlebox, which then notifies the {\ushaper} in the server
%middlebox. The {\ushaper} in the server middlebox initiates a handshake with
%the server on behalf of the remote client. When the handshake with the server is
%complete, the server middlebox responds to the client middlebox, which then
%completes the handshake with the client.

Once the connection is established, each application endpoint may send to the
{\ushaper} in its local middlebox an optional shaping configuration
request, which indicates the choice of DP parameters and/or latency constraints
it wishes to use for shaping its outbound
traffic\footnote{Before forwarding the DP parameters to their respective
middleboxes, the applications run an additional handshake protocol after
connection establishment to negotiate the parameters for the traffic between
them.}.
%
Finally, the {\ushaper} sets up an entry in a local {\flowmap} table to establish
shaping for the application endpoints.
%mapping the three connection segments, the associated socket and per-flow
%transmit and receive queues, and the DP parameters for traffic shaping that were
%provided by the application endpoints at the time of flow registration.
%\am{deduplicate from the overview.}

%\paragraph{End-to-end connection shutdown.}
Closing an end-to-end connection follows a similar process as connection
initiation. The {\ushaper} in each middlebox mediates the connection termination
and removes the connection entry from its {\flowmap} table.
%The {\ushaper} in a middlebox intercepts connection termination handshake
%from a client (or server); the {\dshaper} in the middlebox then relays
%connection termination to the {\dshaper} in its peer middlebox; the {\ushaper}
%process on the peer middlebox terminates connection with the corresponding
%server (or client) and responds to the initiating middlebox, which then closes
%the connection with its local node.
%Finally, both middleboxes remove the connection entry from their local
%{\flowmap} tables.
\fi

\subsection{Components}
\label{subsec:impl-mediation}
\paragraph{UShaper.}
The {\ushaper} mediates the unshaped traffic between one or more local
application endpoints and the {\dshaper} using per-flow transmit and receive
queues.
It implements a transport server (or client) for interfacing with each local
client (or server, respectively) application endpoint\footnote{The {\ushaper}
supports both UDP and TCP endpoints for applications.}.
%The type of the transport endpoint depends on the application's choice of
%transport protocol.
Additionally, it shares a {\flowmap} table with the {\dshaper},
which consists of an entry for each end-to-end flow. Each entry maps the
piecewise connections with
%the associated sockets of {\ushaper} and {\dshaper}, a
the pair of transmit and receive queues to carry the local application's byte
stream, and shaping configurations (\eg privacy descriptor) provided by an
%\todo{(\eg privacy descriptor, tunnel lifetime)} provided by an
application at the time of flow registration.
%The transmit queues of the end-to-end flows mapped to a single tunnel connection
%correspond to the tunnel's buffering queue, on which tunnel's DP guarantees
%rely.

The {\ushaper} receives the outbound traffic from a sender application
and enqueues the byte stream into a per-flow transmit queue shared with the
{\dshaper}.
It also dequeues bytes from a per-flow receive queue, repackages them
into transport packets and sends them to the receiver application.
%It also dequeues QUIC packets from a
%%the corresponding
%per-flow receive queue, discards the dummy frames, repackages the payload from
%the remaining frames into transport packets and writes them to the socket of
%the application flow.

%\if 0
\begin{figure}[t]
    \centering
%    \includegraphics[width=\columnwidth]{figures/schedule.pdf}
    \includegraphics[width=\columnwidth]{figures/schedule5.pdf}
    \caption{{\dshaper} schedule}
    \label{fig:middlebox-schedule}
\end{figure}
%\fi

\paragraph{DShaper.}
%\label{subsec:impl-shaping}
%\am{The description does not match the security spec and will be replaced with
%the alternate text once an implementation satisfying the spec is confirmed.}
%\paragraph{Traffic shaping.}

The {\dshaper} process consists of a {\prepare} thread and a QUIC
worker thread.
The {\prepare} thread instantiates a QUIC client/server to establish
a tunnel with the remote middlebox and implements the DP shaping logic.
%On~the transmit side, {\prepare} examines the number of bytes in each
%per-flow transmit queue, determines the number of bytes to transmit,
On the transmit side, {\prepare} \update{prepares shaped buffers based on DP
measurements of the transmit queues}
and then submits shaped buffers to the QUIC worker.
On the receive size, the QUIC worker transmits ACK frames to the sender
and then decrypts the QUIC packets, extracts the STREAM frames, and copies
bytes (including dummy bytes) from each frame into the appropriate per-flow
receive queue.



%The {\dshaper} implements a thread, named {\prepare}, which instantiates a QUIC
%client/server to establish a tunnel with a remote middlebox, as well as the
%DP~shaping logic. The {\dshaper} links the QUIC library, which implements a
%worker thread that receives shaped buffers from {\prepare} and transmits them as
%one or more QUIC packets.
%\mis{I found this quite difficult to parse and want to suggest
%an alternative,
%but I was not 100\% sure that I understood the implementation well enough
%to get this right, so I'm putting it in a comment.
%The {\dshaper} process consists of a single {\prepare} thread and one
%or more QUIC worker threads.
%The {\prepare} thread both instantiates a QUIC client/serer to establish
%a tunnel with the remote middlebox and implements the DP-shaping logic.
%On the transmit side, {\prepare} examines the number of bytes in each
%per-flow transmit queue, determines the number of total bytes to transmit,
%and then submits DP-shaped buffers to the QUIC worker threads.
%On the receive size, QUIC worker threads rtansmit ACK frames to the sender
%and then decrypt the QUICK packets, extract the STREAM frames, and copy
%bytes (including dummy bytes) from each frame into the appropriateper-flow
%receive queue.
%}

%{\prepare} implements a periodic loop of length $T_{prep}$ that runs until the
%end of the tunnel lifetime.
%{\prepare} implements a while loop that runs until the end of the tunnel
%lifetime, which mainly follows the design from \S\ref{subsec:design-overview} to
%transmit shaped packets.
%After periodic intervals of length $T_{prep}$, it computes a
%differentially-private transmission size $S$ and prepares a transmit buffer of
%the same length to be sent out over QUIC.
%In each loop iteration, it prepares a transmit buffer of a
%differentially-private size $\qlendp$ to be sent to QUIC.
%{{\prepare} iterates through the transmit queues mapped to the tunnel; it
%dequeues a number of payload bytes from the queues that is the minimum of
%$\qlendp$ and the available bytes on the queues and appends them to the transmit
%buffer.}
%If the total number of payload bytes available across all transmit queues is
%lower than $\qlendp$, {\prepare} further appends dummy bytes for the remaining
%length of the transmit buffer.
%Finally, {\prepare} enqueues the transmit buffer to QUIC.

%The QUIC worker generates QUIC STREAM frames using the bytes from the
%appropriate streams passed in the transmit buffer, and then packages the STREAM
%frames into one or more QUIC packets. Finally, {the QUIC worker}
%encrypts the QUIC packet and forwards it to the underlying UDP layer, which
%ultimately transmits the packets at link speed.

%%%%%%%%%%%%%%%%%%%%%%%%%%
%%% Correct implementation
%%%%%%%%%%%%%%%%%%%%%%%%%%
%The {\dshaper} iterates through the transmit queues mapped to the tunnel; it
%dequeues a number of payload bytes from a transmit queue that is minimum of $S$
%and the available bytes on the queue, packages them into a QUIC STREAM frame,
%and appends the frame to the transmit buffer. If the total number of payload
%bytes available across all transmit queueus is lower than $S$, the {\dshaper}
%further enqueues a dummy frame of length $S - P$, where $P$ is the total number
%of payload bytes dequeued from the transmit queues. Finally, the {\dshaper}
%forwards the buffer to QUIC, which encapsulates the buffer into a QUIC packet,
%encrypts it, and then forwards it to the underlying UDP layer, which ultimately
%transmit the packet at link speed.
%At periodic intervals, the Shaper computes a differentially-private transmission
%size $S$, dequeues a number of payload bytes $P$ from the transmit queue, where
%$P$ = $min$($S$, total bytes in queue), and packages them into a QUIC frame. The
%Shaper also prepares a frame with a number of dummy bytes $D$ = $S - P$.
%Finally, the Shaper packages the payload and dummy frames into a single QUIC
%packet, encrypts the packet, and forwards the packet to the underlying UDP
%layer, which ultimately transmits the packet at link speed.

%The {\prepare} and QUIC worker threads follow the design from
%\S\ref{subsec:design-overview} to transmit shaped packets.
%When shaped QUIC packets arrive from a tunnel, QUIC transmits
%an ACK frame as a response to the sender, decrypts the received QUIC
%packets, extracts the STREAM frames, and copies the bytes (including dummy) from
%each frame into the appropriate per-flow receive queues shared with the
%{\ushaper} process.
%The {\ushaper} handles the packets as discussed in
%\S\ref{subsec:impl-mediation}.
%The {\dshaper} decrypts each inbound QUIC packet received from a tunnel and
%places
%the packet in a per-flow receive queue shared with the {\ushaper} process. QUIC
%also transmits an ACK frame as a response to the sender.
%\todo{Note that the ACK frames are themselves not subject to DP shaping.}

\if 0
%%%%%%%%%%%%%%%%%%%%
%% no longer needed?
%%%%%%%%%%%%%%%%%%%%
\paragraph{\todo{Prioritizing payload over dummy.}}
Note that %Recall that
{\prepare}'s payload preparation logic executes once at the beginning of every
interval of length $T_{prep}$.
%, \eg at time $t$, $t + T_{prep}$, $t + 2T_{prep}$, and so on.
Consider a scenario where an application's payload is
enqueued in a transmit queue at a small time $\theta$ after
the {\prepare} thread checked the transmit queue for payload bytes at the
beginning of interval $k$.
%$kT_{prep}$.
%In this case, there is no application data to transmit during the
%interval $[kT_{prep}, (k+1)T_{prep})$.
%{\prepare} will transmit dummy bytes in the interval $[kT_{prep},
%(k+1)T_{prep})$, while the application
%payload will be delayed by at least $T_{prep}$ and will be transmitted during
%the next interval $[(k+1)T_{prep}, (k+2)T_{prep})$.
{\prepare} will transmit dummy bytes in the interval $k$, while the
application payload will be delayed by at least $T_{prep}$ and will be
transmitted during the next interval ${k+1}$.
To reduce the transmission latency for the application, {\sys} modifies the
implementation of {\prepare} such that it can prioritize
payload bytes over dummy bytes more frequently.

{\prepare} implements a higher frequency loop with interval $T_{dequeue}$ inside
the
loop with interval $T_{prep}$. It splits the DP size decision generated at the
beginning of $T_{prep}$ into $T_{prep}/T_{dequeue}$ smaller uniform sizes and
prepares smaller transmit buffers by checking the transmit queue once at the
beginning of every $T_{dequeue}$ interval.
%\am{Revisit based on final design and experiments.}
\fi

%When the {\DPlogic} computes the size for the next burst transmission, it places
%a token in a local {\tokenq} rather than immediately dequeueing bytes from
%{\txq}. The packetizer, which is now decoupled from the {\DPlogic}, periodically
%checks the {\tokenq}. If the {\tokenq} is non-empty, it dequeues payload and
%dummy bytes appropriately from {\txq} to prepare a buffer of size determined by
%the first dequeued token; otherwise, the packetizer goes to sleep.
%
%The intervals of the {\DPlogic} and the packetizer determine a tradeoff between
%transmission latency for payload bytes and the bandwidth overhead due to dummy
%bytes.
%Optimally, the packetizer interval must be smaller than the {\DPlogic} interval,
%while the {\DPlogic} interval must align with the application traffic rate.
%However, the {\DPlogic} interval must not be highly reactive to the application
%traffic rate as it could reveal application secrets.
%In practice, {\sys} would incur low overheads when the traffic has a stable
%burst rate.
%%\todo{TODO}

%\paragraph{Privacy aggregation and flow prioritization.}
%{\sys} allows clients to configure the tradeoff between their individual privacy
%and overheads.
%%In principle, {\sys} provides DP guarantees individually for each application
%%flow.
%In principle, {\sys} can shape each application flow through an independent
%tunnel with per-flow DP guarantees. However, if several application endpoint
%pairs use the same middleboxes as tunnel endpoints, they can choose to amortize
%their overheads by sharing a tunnel and their DP privacy budget.
%%However, clients using the same tunnel can choose to amortize their overheads
%%by sharing their privacy budget.
%Additionally, they may provide a prioritization factor to allow {\sys} to select
%payload bytes from their per-flow queues in order of their priority. Clients can
%notify their middlebox about their desired privacy guarantee and prioritization
%factor using the privacy configuration protocol.
%
%To shape multiple flows through a shared tunnel, a {\dshaper} initializes a
%fixed
%number of data streams in the tunnel connection. When the {\ushaper} receives a
%new
%application flow, it adds a mapping for the application connection, and a pair
%of transmit and receive queues with the shared tunnel connection. Upon receiving
%a privacy configuration message, the {\ushaper} updates the configuration of a
%flow. Subsequently, at each interval, the {\dshaper} process selects payload
%bytes
%by iterating through the per-flow queues belonging to the same privacy class in
%order of the queues' priority.

\subsection{Ensuring Secret-Independent Shaping}
\label{subsec:impl-shaping-security}
%\Cref{fig:middlebox-schedule} illustrates the schedule of operations on
%{\prepare}
%and QUIC worker threads on the outbound path.
%The green and orange boxes represent data-independent and data-dependent
%operations, respectively.
The goal of the middlebox is to ensure that {\em an adversary observes
$\qlendp$ bytes in each transmit interval $\dpintvl$.}

Let's first understand the factors that might prevent the middlebox from
guaranteeing this property.
Even though an application is physically isolated from the middlebox and can
encrypt its data (\eg using end-to-end TLS), its flow control behavior could be
secret-dependent and could affect the middlebox's execution.
For instance, the presence or absence of payload traffic from an application
can affect the time {\dshaper} requires to prepare the shaped buffers.

Ensuring the high-level goal mentioned above requires that
(i) {\prepare} computes $\qlendp$, allocates and prepares a buffer of length
$\qlendp$, and passes the buffer to the QUIC worker within $\dpintvl$,
(ii) the QUIC worker prepares encrypted packets from the buffer and sends them
to UDP, such that the total payload size of the QUIC packets prepared in
$\dpintvl$ is $\qlendp$, and
(iii) the UDP stack transmits the packets totaling to $\qlendp$ bytes of payload
size to the NIC in $\dpintvl$.
Enforcing all these properties would produce a strict time-trigggered schedule
for each component, which would significantly reduce link utilization and
increase packet transmission latencies.
%Moreover, the value of $\dpintvl$ required would be large to account for
%potential secret-dependent (\eg flow control) as well as secret-independent
%delays (\eg congestion control).
%This would significantly increase packet transmission latencies.

{\dshaper} instead provides the following guarantees. (See
\Cref{fig:middlebox-schedule} for reference.)
%The {\dshaper} provides two guarantees.
First, {\prepare} \update{guarantees that a DP measurement $\qlendp$ is performed
every fixed time interval $\dpintvl$}.
Secondly, {\prepare} guarantees that a shaped buffer of length $\qlendp$ is {\em
prepared} within a fixed time $\dpintvl_{prep}$.
Thirdly, {\prepare} locks the shaped buffer for a fixed time,
$\dpintvl_{enq}$, during which it enqueues the shaped buffer for a QUIC
worker.
This ensures that the buffer is completely enqueued before QUIC starts
transmitting it and that
QUIC receives the buffer only at fixed delays.
%\todo{
We empirically profile the time taken by {\prepare} for preparing and enqueueing
shaped buffers for various DP lengths. We set $\dpintvl_{prep}$ and
$\dpintvl_{enq}$ to maximum values determined from profiling, and $\dpintvl$ to
the sum of these maximum values. If {\prepare} takes time less than
$\dpintvl_{prep}$ (or $\dpintvl_{enq}$, respectively) to prepare (or enqueue) a
shaped buffer, it sleeps until the end of the interval before moving to the next
phase.
%}
%\todo{We empirically profile the maximal time $\dpintvl^{max}_{prep}$ and
%$\dpintvl^{max}_{enq}$ taken by {\prepare} for preparing and enqueueing shaped
%buffers for various DP sizes. We set $\dpintvl_{prep} = \dpintvl^{max}_{prep}$,
%$\dpintvl_{enq} = \dpintvl^{max}_{enq}$, and $\dpintvl = \dpintvl^{max}_{prep} +
%\dpintvl^{max}_{enq}$. If {\prepare} takes time less than
%$\dpintvl^{max}_{prep}$ (or $\dpintvl^{max}_{enq}$, respectively),
%to prepare (or enqueue) a shaped buffer,
%it sleeps until the end of the interval before moving to the next
%phase.}
%\am{Too symbol heavy?}


%{\dshaper} instead provides two guarantees.
%%The {\dshaper} provides two guarantees.
%First, {\prepare} guarantees that each shaped buffer is {\em prepared} within a
%fixed time interval $\dpintvl$.
%\todo{For this, we empirically profile the maximal time taken $\dpintvl_{max}$
%by {\prepare} until
%buffer preparation for various DP sizes and set $\dpintvl$ to this
%$\dpintvl_{max}$. If {\prepare} takes lesser time than $\dpintvl_{max}$ to
%prepare a transmit buffer, it sleeps until the end of the interval, at which
%point it starts enqueueing the buffer to QUIC.}
%Secondly, QUIC's packetization remains data-independent. For this, {\prepare}
%synchronizes with the QUIC worker on the the transmit buffers,
%%the preparation of buffers to be transmitted,
%ensuring that QUIC cannot receive fewer bytes than the computed DP
%size of the interval before it sends packets to the network. F

In the middlebox, {\prepare} and QUIC worker threads run on a separate cores
sharing only the shaped buffers.
{\ushaper} runs on yet a differnet core, shares only the
{\flowmap} and the per-flow queues with {\dshaper}.
Variations in {\prepare}'s execution due to the state of the
per-flow queues are hidden by $\dpintvl_{max}$, while QUIC's
execution depends only on shaped buffers and thus, is secret-independent.
Consequently, the packetization of shaped buffers in the QUIC worker and the UDP
stack is secret-independent and any variations in packet transmit times induced
due to their execution constitute post processing noise.

A remaining concern could be leaks via internal side channels in the middlebox
that cause {\dshaper} to fail to prepare the expected amount of data within a
scheduled interval.
For instance, {\dshaper}'s execution could be influenced by microarchitectural
state (\eg caches, memory and PCI buses, write buffers, interrupts) based on the
application's flow control.

\if 0
A remaining concern could be leaks via internal side channels in the middlebox
that cause {\sys} to fail to transmit the expected amount of data within a
scheduled interval. Even though an application is physically isolated from the
middlebox and may encrypt its data (\eg using TLS for the end-to-end
connection), the application’s flow control could be secret-dependent and could
affect {\sys}'s execution.

\todo{For instance, flow control affects the number of payload bytes available
for transmission and, consequently, the amount of padding that may be added to a
segment. Processing payload and dummy bytes could take different amounts of
time.} Secondly, the execution of the Shaper could be influenced by interrupts
or microarchitectural state (\eg caches, memory and PCI buses, internal write
buffers) based on the presence or absence of payload traffic from the
application.
\fi

We have not been able to exploit such side channels to identify traffic content.
Nevertheless, such side channels could be eliminated via resource partitioning,
performance isolation, and constant-time implementation techniques
\cite{liu2016catalyst, coppens2009practical, zhang2011predinteractive,
    almeida2016verifying}.



\subsection{Scheduling Across Tunnels}
{When transmitting traffic on multiple tunnels, {\sys} must ensure that the
unshaped traffic of one tunnel is not leaked to another tunnel. For this, {\sys}
must isolate the tunnels from each other in the middlebox.
%Based on \S\ref{subsec:impl-shaping-security}, we require that the {\prepare}
%and QUIC worker threads must be performance isolated from {\ushaper} in each
%tunnel, (ii) the timing of {\prepare} must be masked to secret-independent
%times.
Thus, {\sys} partitions the middlebox cores into three groups, each core group
hosting the {\ushaper} process, the {\prepare} threads, and the QUIC worker
threads from different tunnels.
Furthermore, {\sys} uses a TDMA schedule among the {\prepare} threads, while
\update{padding} each thread's execution to a secret-independent time.
%In {\sys}, only the {\dshaper} components need to be isolated. {\sys} uses a
%TDMA to schedule the {\dshaper} processes of different tunnels.
Since each {\prepare} thread enqueues shaped buffers at secret-independent
times, the QUIC workers can subsequently package the buffers into packets and
transmit the packets across multiple tunnels following any arbitrary schedule.}
%
{Determining optimal TDMA schedules and their adaptation to the changing
number of active tunnels is left to future work.}

\if 0
%\paragraph{Shaping outbound traffic.}
\subsection{Reliable Delivery}
\am{Explain how this is relevant to security.}
Applications relying on TCP expect reliable delivery guarantees. Thus, {\sys}'s
middlebox needs to support flow control, congestion control, and loss recovery
to enable reliable delivery across the piecewise connections.

%\paragraph{Between an end host and a middlebox.}
For a connection between an end host and the middlebox, flow control, congestion
control, and loss recovery are handled by the transport layer protocol used on
the connection as usual.
%
%\paragraph{Between two middleboxes.}
For a tunnel connection, the QUIC protocol handles flow control, congestion
control, and loss recovery in
the tunnel.
%In case of congestion or packet losses on the network carrying the tunnel
%traffic,
QUIC buffers the prepared outbound packets until they are acknowledged and
retransmits unacknowledged packets in case of packet losses. The buffered
packets contain traffic whose size and timing have been shaped; therefore,
additional delays due to network congestion or packet losses only add noise to
an adversary’s observations and do not affect application’s privacy.

%\paragraph{Impact of prolonged network instability.}
In case of prolonged congestion or losses, or if the receiver is overwhelmed for
an extended period of time, QUIC's buffers in the sender middlebox may overflow
and drop packets.
The sender middlebox must then apply a back pressure on its local end hosts to
force them into slowing down their transmissions. MinesVPN’s middlebox
implements the back pressure mechanism as follows. When the {\dshaper}'s QUIC
buffer overflows, it stops dequeueing payload bytes from the per-flow transmit
queue. This causes the transmit queue to fill up and prevents the {\ushaper}
from enqueueing more bytes into the queue, which in turn causes the {\ushaper}
process to not read bytes from the TCP socket interfacing with the application.
Consequently, TCP notifies the sender of a reduction in the receive window
causing the sender to slow down transmission. Eventually, TCP's buffers may fill
up and cause TCP to drop incoming packets from the application, ultimately
notifying the sender application's TCP stack of congestion.

The system recovers from congestion once {\dshaper} receives
acknowledgements for transmitted packets and can dequeue payload
bytes from the transmit queues\footnote{{\sys} could expedite congestion
notification to the sender application by using mechanisms, such as explicit
congestion notification \cite{ecn}. We leave a detailed analysis of congestion
handling to future work.}.

A remaining challenge arises when a sender middlebox acknowledged payload bytes
from the local sender application, but is forced to drop the bytes due to
instability on the tunnel network. This violates the reliable delivery semantics
expected by the application. Note that existing proxies face a similar challenge
too. {\sys} does not aggravate the issue and, therefore, similar to other
proxies, leaves the resolution to the application and the user.
%\am{Dealing with bytes acknowledged by middlebox but no longer able to buffer.}
%\todo{Recovery from congestion.}
\fi

%\subsection{Scheduling across tunnels.}
%Once the traffic within each tunnel is shaped, sending and receiving traffic
%across multiple tunnels can follow any schedule.





%%%%%
%%%%%
\if 0
The middlebox consists of two VMs: host-facing ({\unshapedVM}) and
tunnel-facing ({\shapedVM}). Each VM hosts a separate network stack, which
consists of a transport layer on top of a
network layer on a top of an ethernet layer. The {\unshapedVM} supports one or
more transport protocols, such as TCP, UDP, and QUIC.
The {\shapedVM} primarily relies on UDP but additionally runs three layers atop
UDP: a {\DPlogic} on top of an encryption layer, which is integrated with the
QUIC protocol~\cite{langley2017quic}\footnote{In principle, the {\shapedVM} could use
TCP as a
    reliable tunnel transport; however, we choose QUIC for \todo{reasons of efficiency and
        ease of implementation}.}.
%because it enables efficient multiplexing of multiple client streams, avoids
%head-of-line blocking,

The {\unshapedVM} receives unshaped traffic from an
end-host application and forwards it to the {\shapedVM}. The {\DPlogic} shapes
the traffic according to DP and transmits it over a QUIC connection. In the
reverse direction, the {\shapedVM} forwards the traffic received over the QUIC
connection to
the {\unshapedVM}, which in turn forwards it to the target application after
decryption and removing any padding.

We now elaborate on the interaction between an end-host application and a
middlebox, as well as the components of the middlebox.

\subsection{\unshapedVM}
%
%The {\unshapedVM} places an application's outbound bytes, including handshake
%and control packets, in the transmit queue, which are dequeued and shaped in the
%{\shapedVM}. Similarly, the {\shapedVM} places inbound packets from the tunnel
%in the receive queue, which are dequeued in the {\unshapedVM}, decrypted,
%stripped of padding, and forwarded to the appropriate end-host application.

The {\unshapedVM} contains a userspace application,
called the {\mediator}, and a small kernel module, which interact via another
FIFO queue in a shared memory region.
The kernel module maintains the {\flowmap}, which consists of the
mapping of the segments of each end-to-end connection and other configuration
parameters for the connection.
In addition, the {\mediator} interfaces with the {\shapedVM} via statically sized lockfree FIFO
queues. For each end-to-end connection, there is a pair of transmit and receive
queues allocated in a shared memory region between the VMs.

When the middlebox receives a new flow from an end host application, the kernel
module in the {\unshapedVM} intercepts the handshake messages, copies them into
the FIFO queue shared with the {\mediator} and responds to the end host in
accordance with the transport protocol.  The {\mediator} forwards the handshake
messages to the {\shapedVM}, which handles the remaining stages of the
end-to-end connection establishment with the remote peer and returns information
of the later connection segments to the {\mediator}. The {\mediator} forwards
the connection information to the kernel module, which then populates a
{\flowmap} entry for the end-to-end connection.

Once a connection is established, the kernel module also intercepts the data
packets of the end host's transport protocol, copies them into the FIFO queue
shared with the {\mediator}, and sends appropriate responses to the end host in
accordance with the transport protocol.
Furthermore, the {\mediator} decrypts packets from the receive queue, strips off
any padding, and forwards the payload bytes to the kernel module. The kernel
module encapsulates the payload with protocol headers and forwards
the packets to the appropriate end hosts.

\subsection{\shapedVM}
The {\shapedVM} implements the core of {\sys}'s traffic shaping design.
The {\shapedVM} establishes a bidirectional QUIC connection with the
{\shapedVM} in each of its peer middleboxes. Within each connection, the
{\shapedVM} further opens a \todo{bidirectional} QUIC stream with its peer,
which is assigned the stream ID 0 and is used as a stream for dummy byte
transmissions.
\todo{TODO: Complete the section}
\fi

%\begin{figure*}[t]
%\center{
    %%    \centering
    %    \subfigure[Time line of connection establishment in {\sys}] {
        %%    \includegraphics[width=\columnwidth]{figures/connection-establishment.pdf}
        %    \includegraphics[width=\columnwidth]{figures/conn-est.pdf}
        %    \label{fig:connection}
        %    }
    %%\end{figure}
    %%\begin{figure}[t]
    %%    \centering
    %    \subfigure[Time line of connection termination in {\sys}] {
        %%    \includegraphics[width=\columnwidth]{figures/connection_termination.pdf}
        %    \includegraphics[width=\columnwidth]{figures/conn-term.pdf}
        %    \label{fig:termination}
        %    }
    %}
%\caption{Foo}
%\end{figure*}
%


==> overview.tex <==
\section{Overview}
\label{sec:overview}


%Protecting clients' privacy requires ensuring confidentiality of their network
%traffic content.
%The content may be leaked through the traffic shape, \ie, the packet sizes,
%inter-packet intervals, and the direction of the traffic. Additionally, it may
%be leaked through the time of a client's initiation of communication with a
%service, and the duration of the communication.
%\todo{In applications where the traffic passes through multiple nodes on the
%Internet, the content may additionally be correlated with the sequence of
%interactions with the nodes, which constitute a traffic DAG (directed acyclic
%graph).}

%\am{Describe a real-world motivating example.}

A secure and practical {\nsca} mitigation system must satisfy the following
design goals:
{\bf G1.} Address leaks through all aspects of the shape of transmitted traffic,
{\bf G2.} Provide quantifiable and tunable privacy guarantees for the
communication parties,
{\bf G3.} Minimize overheads incurred while guaranteeing privacy,
{\bf G4.} Support a broad class of applications, and
{\bf G5.} Require minimal changes to the applications.
%{\bf G5.} Enable tuning between privacy guarantees and overheads with minimal
%changes modifications to the applications. {\as{Maybe we can combine G5 and G3}}

{\sys}'s shaping prevents leaks of the traffic content through sizes, timing,
and direction of packets \todo{along all communication links between application
nodes} (G1).
%\todo{It can also hide the precise times of network activity.} (G1).
%
We present the key ideas of {\sys}'s shaping that help achieve the remaining
goals. We then present {\sys}'s threat model.
%We present the key ideas of our solution that help achieve the above goals and
%the threat model and assumptions we are operating on.
%We start by listing the key goals for designing a {\nsca} mitigation system. We
%then describe the threat model and assumptions we are operating on, and finally
%the key ideas of our solution.

%\subsection{Design goals}
%\label{subsec:goals}
\subsection{Key ideas}
\label{subsec:key-ideas}

\paragraph{Differentially private shaping.}
%Ensuring confidentiality of content requires shaping the
%packet sizes and timing along all links involved in a client's network traffic.

%A strawman approach is constant shaping, which would require continuously
%transmitting fixed-length packets with a fixed inter-packet interval.
%Constant shaping is a secure approach, but can induce significant bandwidth and
%latency overheads. Prior work has proposed ways to allow variations in traffic
%shaping that reduce overheads at the cost of privacy leaks.
%\todo
As discussed in \S\ref{sec:intro}, unlike constant shaping and
variable-but-static shaping, dynamic shaping offers the most flexibility for
adapting traffic shape at runtime based on workload patterns and, therefore, can
reduce significantly reduce overheads.
%Dynamic shaping can help to reduce costs of mitigating network side channels at
%the cost of some privacy leak.
{Unfortunately, existing dynamic shaping techniques either have unbounded privacy
leaks or offer only weak privacy guarantees.
%Moreover, some of these techniques require extensive profiling of an
%application's network traffic traces.
}
%\am{Check recent techniques.} \am{How can we compare privacy
%leakage of k-anonymity vs differential privacy?}{\as{I think k-anonymity has
%$\varepsilon$ of infinite as the output probability for any two trace from two
%different groups of anonymity is not bounded.}}
%
%{\sys} instead relies on a dynamic shaping technique that provides
%%allows variations in traffic shapes while providing
%%\todo
%{quantifiable privacy leaks with tunable bounds} and without requiring
%extensive pre-profiling of application traffic.
%%\todo{{\sys}'s shaping hides the time of initiation and termination of
%%transmissions}, as well as the content of the transmissions (G1).
%Specifically, {\sys} provides differential privacy guarantees in its shaping
%(G2).
%Specifically, it generates differentially-private burst length for transmission
%in periodic intervals.
{\sys}'s \todo{novel} differential privacy (DP) based shaping strategy provides
quantifiable privacy leaks with tunable bounds and without relying on profiling
of application traffic (G2).
\todo{The DP guarantees are determined on fixed-length burst intervals and
composed across consecutive intervals to quantify the overall privacy
guarantees for an application.}
%\am{\ml{@Mathias: verify if the above English explanation of the DP guarantees
%is accurate.}}
%
%{\sys}'s shaping incurs lower overheads compared to constant shaping as well as
%other prior techniques (G3).
%We discuss the shaping technique in \S\ref{sec:dp} and evaluate its performance
%in \S\ref{sec:eval}.

\paragraph{Shaping in a middlebox.}
%\S\ref{fig:minesvpn-overview} provides an overview of {\sys}'s architecture.
{\sys} relies on the abstraction of a tunnel for implementing traffic shaping.
Application traffic is shaped between the tunnel endpoints such that an
adversary observing the tunnel traffic cannot infer application secrets.
In principle, a tunnel endpoint could be integrated with the end host hosting an
application (\eg in a VM isolated from the end-host application), or in a
separate node through which the application's traffic passes.
{\sys} relies on the second approach and implements the tunnel endpoint as a
middlebox, which could be integrated with an existing network element, such as a
router, a VPN gateway, or a firewall.
%(see \S\ref{sec:implementation} for more details).
The middlebox implementation enables securing multiple applications without
requiring modifications on individual end hosts (G4).
Furthermore, for multiple flows that require the same tunnel, it allows pooling
the flows under the same privacy guarantees, which helps to amortize the
per-flow overhead (G3).
%We elaborate on the {\sys}'s implementation in \S\ref{sec:implementation} and
%evaluate the performance optimization in \S\ref{sec:eval}.
%\ml{Here we need to emphasize that sharing a pipe is very good for privacy
%guarantees (assuming we evaluate it? To me that's a core benefit of the
%middlebox deisgn so it'd be really good to have it.) Maybe something like
%``Importantly, our middlebox design enables pooling multiple clients through
%the same protected tunnel, providing privacy guarantees to mulitiple
%connections at a fixed overhead (\S\ref{sec:dp}).''}

\paragraph{Minimal modifications to end applications.}
%\todo{TODO.}
By default, {\sys} shapes all traffic through a tunnel with a fixed differential
privacy guarantee, \ie with a single value of $\epsilon$ and $\delta$. However,
an application can explicitly specify its privacy requirements ($\epsilon$ and
$\delta$), as well as
bandwidth and latency constraints, and any prioritization preferences on a
per-flow basis to its local middlebox. This requires small modifications in the
application to transmit a shaping configuration message to the middlebox along
with the application flow. Thus, {\sys} offers a balance between being fully
application-agnostic versus optimizing for privacy or overhead with minimal
support from the applications (G2, G5).
%\am{We need to know how {\sys} should use DP parameters for 5s intervals or for
%sensitivity of 2MB.}

\subsection{Threat Model}
\label{subsec:threat-model}
%{\sys}'s goal is to protect an application's secrets from being leaked to a
%network adversary.
%We assume that the communicating nodes are inside a trusted private network,
%\eg behind a VPN gateway node, which an adversary cannot compromise.
%\todo{We assume that all the application endpoints are non-malicious and do not
%explicitly leak the secrets themselves. The secrets could be leaked only through
%side channels. A service serving both privacy-sensitive and privacy-insensitive
%clients is partitioned into two instances, with each instance dedicated to
%serving clients with similar privacy requirements. For the privacy-sensitive
%clients, we assume the corresponding service endpoint agrees to serve the
%clients according to their privacy requirements.}

%{\sys}’s goal is to protect an application’s secrets from being leaked to a
%network adversary.
{\sys}'s goal is to hide the content of an application's network
traffic.
%\todo{as well as the time of initiation and the duration of the network
%activity}.
%\am{Despite the ``always-on'' tunnels, we still have coarse-grained leaks of
%start times of flows when a flow selects different DP parameters than default.
%If we further imagine starting tunnels just before transmissions, such as for a
%multi-hop scenario, we should not talk about hiding initiation times.}
We assume that the communicating nodes are inside separate trusted private
networks (\eg each node is behind a VPN gateway node), which an adversary
cannot compromise. We assume that all the application endpoints are
non-malicious and do not leak the secrets themselves.
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% can handle non-sensitive traffic simultaneously by just using TDMA
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%Furthermore, we assume that applications transmitting only non-sensitive
%traffic are partitioned from the applications transmitting sensitive traffic.
%For instance, the non-sensitive applications use a different router.

%We assume that the communication between all nodes in the client's traffic DAG
%is encrypted.
The adversary controls network links in the public Internet (\eg ISPs) and can
record, measure, and tamper with the victim's traffic as it traverses through the
links under the adversary's control.
In particular, it can precisely record the traffic shape---the sizes, timing,
and direction of packets---on all links in the victim's traffic
\todo{communication graph}.
Furthermore, the adversary can drop, replay, or inject packets into the victim's
traffic.
However, it cannot break standard cryptography, cannot compromise the victim's
VPN, or cannot impersonate its clients or servers to directly interact with the
victim \update{(thus, no covert attacks).}
\update{We do not consider threats due to observing the IP addresses of packets,
although {\sys} can hide IP addresses of application end hosts behind a shared
traffic shaping tunnel.}
%We also do not consider the threat where an adversary colocates with
%the victim inside the victim's private network to observe the victim's traffic
%shape through indirect contention signals~\cite{mehta2022pacer}.
We also do not consider the threat where a victim accidentally installs a
malicious script in the browser, thus enabling an adversary to colocate with the
victim's application and observe its
traffic~\cite{schuster2017beautyburst,mehta2022pacer}.  This is a reasonable assumption,
since a colocated adversary can exploit many other direct or indirect channels
for data leaks that will be far more efficient than
{\nsc}s~\cite{kocher2018spectre, yarom2014flushreload, liu2015llcpractical, irazoqui2015ssa, vila2017loophole}.
%\eg by renting a VM or by installing a malicious script from a malicious website
%enticing the victim to accidentally install malicious scripts from a malicious
%website.
%\todo{TODO: how do we handle victim accidentally visiting malicious websites and
%installing malicious javascript, etc. on its device? In other words, how do we
%completely rule out colocated adversary?}

%\todo{TODO: Describe the assumptions on adversary knowledge or capability w.r.t.
%differential privacy.}

In this paper, we focus on an implementation of {\sys}'s traffic shaping tunnel
within a middlebox that can be placed in front of the gateway router of an
organization.
%We discuss implementation alternatives in \S\ref{sec:discussion}.
%
{\sys}'s trusted computing base (TCB) includes all components in the
organization's private network and the middleboxes. We assume
that the middleboxes do not directly leak application secrets to the adversary.
In practice, bugs or vulnerabilities in the middleboxes could be eliminated
using standard techniques, such as software fault isolation~\cite{tan2017sfi}. We
assume the cryptographic libraries are side-channel
free~\cite{almeida2016verifying}.
%\todo{{\sys} prevents leaks of applications' secrets via side channels within its
%    middleboxes, such as timing and microarchitectural side channels (see
%    \S\ref{sec:implementation}).}

{\sys} does not address leaks of one application's sensitive data through the
traffic shape of colocated applications transmitting only non-sensitive traffic.
Such leaks may arise, for instance, due to microarchitectural interference among
the applications colocated on a host or among their flows if they pass through
shared links. Mitigating such leaks would require physically isolating the
applications and their flows. For instance, a service serving both
privacy-sensitive and privacy-insensitive clients may be partitioned into two
instances, with each instance dedicated to serving clients with similar privacy
requirements. For the privacy-sensitive clients, we assume the corresponding
service instance agrees to serve the clients according to their privacy
requirements. Alternatively, end hosts could implement mitigations for various
side channels to support colocated applications \cite{mehta2022pacer,
page05partitionedcache, shi2011limiting, kim2012stealthmem,
varadarajan2014scheduler, braun2015robust}. To mitigate leaks among colocated flows at shared
links, {\sys} assumes that the network paths of the sensitive and non-sensitive
flows are completely partitioned. In practice, this limitation can be removed by
combining {\sys}’s traffic shaping with TDMA scheduling \cite{beams2021ifs,
vattikonda2012tdma}.

{\sys} does not prevent leaks of applications' secrets via side channels, \eg
microarchitectural side channels, in its middleboxes. We discuss potential
mitigations in \S\ref{subsec:impl-security}.

\update{Under these assumptions, {\sys} prevents leaks of application secrets
%\todo{and the timing of network activity}
through the sizes and the delays between the network packets transmitted in
either direction between the application endpoints.}
%\todo{Although anonymity is not the focus of our work, {\sys} hides the number
%and identity of the participants communicating between two sites.}

%\update{Under these assumptions, {\sys} prevents leaks of application secrets
%through the sizes of the network packets, the inter-packet intervals, the time
%of initiation of a network activity, or the duration of network activity in
%either direction of communication between the application endpoints.}

